Are Web Agents Still Detectable? Stress-Testing Bot Defenses with Coordinated Evasion

AI web agents can autonomously navigate websites and complete various tasks. As their capabilities and adoption expand, evaluating bot defenses requires adversarial stress tests. Although prior work demonstrates that existing agents can remain detectable, it remains unclear how effective bot defenses are against adversaries that coordinate evasion across browser fingerprints, automation controls, and interaction behavior. To investigate this threat, we introduce DarkAgent, an autonomous web agent that combines a forked Chromium browser that conceals automation artifacts and generative models that produce human-like mouse and keyboard traces. To address the limitations of existing keyboard mimickers, our keyboard model jointly generates realistic key events and their timings while reliably reproducing the target text. Released agent detectors accept our generated behavior as human, and trained classifiers find it substantially harder to distinguish from human traces than existing mimickers. DarkAgent achieves an 89% page-access bypass rate across a third-party stealth benchmark, exceeding the strongest published baseline by 12 percentage points. To further enhance the measurement of agents, we introduce a benchmark that measures browser fingerprints, interaction behavior, and network activity to assess each channel's contribution to detecting adversarial agents such as DarkAgent. On this benchmark, browser and behavioral modifications are complementary: either alone remains detectable, and only their combination evades all tested checks. Together, our findings expose the gap between passing existing bot defenses and reproducing human behavior, and point to timing between actions as a remaining signal for defenders.

==> appendices/ethical-considerations.tex <==
% \section{Ethical Considerations}
% \label{app:ethics}

% \noindent\textbf{Dual-use risks and benefit--harm assessment.}
% Our stakeholders include website operators, legitimate users whose access
% anti-bot gates mediate, security vendors whose protections we evaluate,
% participants in the public interaction corpora we analyze, and defensive
% researchers. Studying coordinated evasion carries clear dual-use risk: a
% browser that suppresses automation artifacts paired with human-trained motor
% generators could lower the cost of unauthorized scraping, credential stuffing,
% bulk account creation, or automated fraud. Secondary risks include unintended
% traffic load on live websites during measurement and biometric re-identification
% in human interaction logs.

% We weighed these risks against the defensive harm of evaluating bot detectors
% only against uncoordinated baselines. Released detectors (\FPAgent and
% AgentShield) report near-perfect accuracy on default agents, yet our
% measurements show that coarse interaction counts and host-specific fingerprints
% fail against heuristic or generative mimicry and unseen execution hosts.
% Documenting these failure modes at the architectural level helps defenders
% audit and harden multi-channel detection. Releasing \MimicTrace alongside
% concrete cross-channel, runtime, and boundary-timing checks while withholding
% turnkey offensive tooling keeps a deployable evasion stack out of public
% circulation.

% \noindent\textbf{Controlled testbed isolation.}
% All component comparisons ($540$ sessions in Table~\ref{tab:matrix}),
% server-verified form evaluations ($40$ live trials in Tables~\ref{tab:agentshield}
% and~\ref{tab:mimictrace-summary}), and multi-channel audits ($172$ honeysite
% sessions and $14$ stock-browser controls in Table~\ref{tab:mimictrace-channels})
% ran exclusively on synthetic web services hosted on our own local infrastructure.
% These experiments created no third-party accounts, conducted no transactions,
% collected no external user data, and kept CAPTCHA solving disabled on the
% honeysite.

% \noindent\textbf{Live-site evaluation.}
% Before testing any live website, we sought sanctioned vendor evaluation
% environments. In August~2026, we contacted DataDome, Kasada, Akamai, and Shape
% to request research testbeds or authorized evaluation access and received no
% response. Without a sanctioned testbed, we ran the public 80-task Stealth
% Bench~V1 suite~\cite{stealthbenchv1} once on August~21, 2026, as it already
% benchmarks commercial browser providers on public pages and provides the only
% reproducible external reference for deployed defenses. Every task was capped at
% a single run and limited to unauthenticated browsing open to any visitor (site
% search, opening a public page, and reading a link). When a site presented a
% CAPTCHA or interactive challenge during that attempt, the agent interacted with
% it within the single task run. The agent logged into no accounts, submitted no
% forms beyond public search queries, made no purchases, posted no content, and
% retained no scraped site content; our analysis records only the binary block
% outcome per task.

% \noindent\textbf{Vendor disclosure.}
% Following our evaluation, we notified the contacted anti-bot vendors with an
% aggregate summary of our Stealth Bench~V1 access outcomes and technical
% descriptions of the evasion mechanisms relevant to their products (out-of-renderer
% control, world-gated observation, native input delivery, cross-channel persona
% alignment, and generative mouse/keyboard synthesis), together with the
% runtime and boundary signals that remained informative in our audit, without
% distributing turnkey patches or exploit code. We remain available to coordinate
% technical follow-up with any vendor that responds prior to publication.

% \noindent\textbf{Human data.}
% We collected no new human-subjects data in this study. Our behavioral models
% train and evaluate exclusively on publicly released corpora used under their
% published terms: the Bo\u{g}azi\c{c}i Mouse Dynamics
% Dataset~\cite{kilic2021bogazici}, the Aalto free-text keystroke
% corpus~\cite{dhakal2018typing}, and the Attentive Cursor
% Dataset~\cite{leiva2020attentive}. \MimicTrace's human reference records come
% from the publicly released logs of \FPAgent~\cite{wang2026fpagent} and
% AgentShield~\cite{agentshield}, from which we derive features solely over their
% recorded fields without pooling unrelated corpora or attempting participant
% re-identification. Only aggregate statistics and anonymized session summaries
% are reported.

% \noindent\textbf{Release policy.}
% While Section~\ref{sec:darkagent} describes the full \DarkAgent, \Browsium, and
% \Behavium architectures so defenders can evaluate and build countermeasures
% against them, we restrict artifact release to prevent turnkey misuse: we
% publicly release \MimicTrace and all defensive measurement and evaluation code,
% while withholding deployable attack code, source-level \Browsium stealth
% patches, trained \Behavium generator weights, and operational attack
% configurations (Appendix~\ref{app:open-science}).



\section{Ethical Considerations}
\label{app:ethics}

\noindent\textbf{Risks and benefits.}
\DarkAgent could facilitate unauthorized scraping, credential stuffing,
bulk account creation, and fraud, harming website operators and users
through privacy violations, financial loss, and increased service costs.
Our results make misuse credible but do not estimate its likelihood or
scale. They also expose limitations in detecting coordinated browser and
behavioral adaptation, motivating stronger defensive evaluation.
We will release \MimicTrace while withholding operational \DarkAgent
artifacts. This reduces direct enablement but cannot prevent reconstruction
from the paper or adversarial tuning against the benchmark. We judge the
benefits of independent defensive evaluation to outweigh these residual risks.

\noindent\textbf{Controlled experiments.}
Component comparisons, form-completion trials, and multi-channel audits
(Tables~\ref{tab:matrix}, \ref{tab:agentshield},
\ref{tab:mimictrace-summary}, and~\ref{tab:mimictrace-channels})
ran on synthetic services hosted on our own infrastructure. They created no
third-party accounts, conducted no transactions, and collected no external
user data. CAPTCHA solving remained disabled on the honeysite.

\noindent\textbf{Live-site evaluation.}
In August~2026, we requested research testbeds or authorized access from
DataDome, Kasada, Akamai, and Shape, receiving no response. These requests
did not establish authorization. To measure deployed access decisions
unavailable in our controlled experiments, we ran the 80-task Stealth Bench~V1
suite~\cite{stealthbenchv1} once on August~21, 2026, with one run per task.
Tasks involved unauthenticated browsing and public searches, including
interaction with challenges encountered during the run. The agent logged
into no accounts, submitted no forms beyond search queries, made no
purchases, and posted no content. We retained binary block outcomes, not
scraped site content. These restrictions reduced potential harm but did not
eliminate the ethical risks of testing without explicit operator consent.


\noindent\textbf{Human data and privacy.}
We use public Bo\u{g}azi\c{c}i~\cite{kilic2021bogazici},
Aalto~\cite{dhakal2018typing}, and Attentive
Cursor~\cite{leiva2020attentive} datasets under their published terms,
with human reference logs from \FPAgent~\cite{wang2026fpagent} and
AgentShield~\cite{agentshield}. We neither link participants across datasets
nor attempt re-identification. Because behavioral traces may remain
identifying after direct identifiers are removed, released data will undergo
privacy and redistribution review. We will document exclusions and provide
acquisition instructions for restricted third-party data where permitted.


\noindent\textbf{Defensive mitigation.}
\MimicTrace's cross-channel, runtime, and boundary-timing checks support
complementary detection. Defenders should validate them on unseen clients
and tasks, combine them with rate limits and account-level controls, and
assess false positives, privacy, and accessibility. 



==> appendices/open-science.tex <==
% \section{Open Science}

% During review, the submission artifact will provide an anonymized repository;
% after de-anonymization, the same materials will be released through a public
% GitHub repository and companion GitHub Pages application. The repository will
% contain the controlled websites, execution validators, task definitions,
% evaluation orchestration, prompts and model budgets, environment manifests,
% preprocessing code, and statistical-analysis scripts for all reproducible
% non-commercial experiments. It will pin source commits, dependency versions,
% detector configurations, random seeds, feature definitions,
% dataset-specific split manifests, model hyperparameters, and checkpoints.
% The split manifests identify the grouping actually used: verified
% participant identities where available, and persistent browser
% identifiers for the \FPAgent data when participant mappings are
% unavailable.
% Per-trial CSV/JSON outcomes will accompany every reported controlled result with a manifest linking each table cell to its source
% artifact. The web application will expose aggregate tables, experiment
% metadata, and links to the corresponding code and results.

% Detector artifacts will be redistributed only when their licenses permit;
% otherwise the repository will provide retrieval and configuration instructions.
% Commercial systems and human traces that cannot be released will be documented
% with sufficient metadata, aggregate outcomes, and justified restrictions. Any
% withheld \DarkAgent component will be listed explicitly with the ethical,
% licensing, or misuse rationale for the omission.

\section{Open Science}
\label{app:open-science}

For artifact inquiries, contact Parsa Nilforushan
at \href{mailto:parsa_nilforushan@sfu.ca}{\nolinkurl{parsa_nilforushan@sfu.ca}}.


==> figures/behavium.tex <==
\begin{figure*}[t]
    \centering

    \subfloat[\KeyboardGen.\label{fig:keyboardgen}]{%
        \includegraphics[width=\textwidth]
            {figures/KeyboardGen_Architecture.pdf}%
    }

    \par\medskip

    \subfloat[\MouseGen.\label{fig:mousegen}]{%
        \includegraphics[width=\textwidth]
            {figures/MouseGen_Architecture.pdf}%
    }

    \caption{\textbf{Behavioral generation in \Behavium.}
    (a) \KeyboardGen generates physical key events followed by timing
    gaps, coupling both decoders through a shared latent.
    Event masks enforce physical legality, while exact target-text
    reproduction and release of all keys define successful generation.
    (b) \MouseGen autoregressively generates timing and spatial
    increments conditioned on the movement request and trajectory
    history. Sampling constraints enforce valid movements and exact
    target arrival, while reconstructed paths are checked for viewport
    containment.}
    \label{fig:behavioral-generation}
\end{figure*}


==> sections/mimictrace.tex <==
\section{\MimicTrace: Multi-Channel Benchmark and Audit}
\label{sec:mimictrace}



Section~\ref{sec:evaluation} showed that each existing evaluation observes one
channel and misses what the others would catch. Stealth Bench~V1 records only
a binary access verdict~\cite{stealthbenchv1}, \FPAgent omits pointer
kinematics and rollover timing~\cite{wang2026fpagent}, AgentShield omits
network and browser telemetry~\cite{agentshield}, and standalone motor corpora
lack a browser runtime~\cite{dhakal2018typing,kilic2021bogazici}. A defender
who observes all channels simultaneously can also test whether they agree with
one another. \MimicTrace provides a self-hosted server, a canonical JSONL
schema (\texttt{mimictrace.session.v1}), and a multi-channel audit that record
network, browser, automation-control, and behavioral telemetry alongside
server-verified task completion.

\subsection{Tasks, Schema, and Dataset}
\label{sec:mimictrace-schema}
\label{sec:mimictrace-cohorts}

\noindent\textbf{Tasks and schema.}
\MimicTrace serves two local task families behind a shared collector and
receipt validator: \emph{interactive browsing} (\texttt{/browsing}, modeled on
\FPAgent~\cite{wang2026fpagent}) and \emph{static/conditional forms}
(\texttt{/forms/simple}, \texttt{/forms/dynamic}, matching
AgentShield~\cite{agentshield}). Matching the published tasks lets us compare
against their released human baselines without collecting new human traces.
Each session logs four synchronized blocks: \textbf{network} (HTTP version,
wire-order header names, \texttt{User-Agent}, \texttt{Sec-CH-UA*}, JA4,
JA4DB); \textbf{browser and control} (navigator, WebGL, Canvas, audio, screen,
and locale attributes, \texttt{navigator.webdriver},
\texttt{document.hasFocus()}, and \texttt{Event.isTrusted}); \textbf{mouse and
scroll} (coordinates, press--release pairs, wheel deltas, speed, acceleration,
button hold, and pre-click pause); and \textbf{keyboard and form timing} (key
events with rollover, paste/\texttt{input} counts, and field-reaction
latencies). Packaging redacts \texttt{Authorization}, \texttt{Cookie},
\texttt{Set-Cookie}, and forwarding headers while keeping wire header order,
and scrubs IP and vendor identifiers.

\noindent\textbf{Dataset and splits.}
The packaged archive holds 690 sessions: 510 browsing sessions across 17
archived stacks ($30$ each) and 180 form sessions ($30$ paired baseline runs on
\texttt{tracker.js} plus $150$ released AgentShield sessions: $11$ human
references and $139$ default agents across $8$ \texttt{simpleForm} and $6$
\texttt{dynamicForm} stacks), alongside $10$ pause-calibrated \MouseGen form
runs ($190$ form sessions total; Table~\ref{tab:mimictrace-summary}). Agent
sessions reside in \texttt{test}; the $11$ human sessions (six authors across
four source-address groups) split into \texttt{train} ($8$) and
\texttt{calibration} ($3$) for frozen-detector evaluation and
permutation-tested C2ST. We do not pool \FPAgent's $546$ human browsing
sessions or the Bo\u{g}azi\c{c}i and Aalto corpora into the form negative
class, because tasks and recorders differ ($>40$\,ms throttled vs.\
packetized) and a classifier would learn the recorder rather than the agent.


\subsection{Behavioral Channel: Matched-Task Form C2ST}
\label{sec:mimictrace-evaluation}

\noindent\textbf{Keyboard and pacing views.}
To test whether form sessions that pass frozen AgentShield remain separable on
the same task, we run a matched-task XGBoost classifier two-sample test
(C2ST)~\cite{lopezpaz2017c2st} ($20\times$5-fold CV, 200-shuffle permutation
nulls) across \textbf{Keyboard} ($10$ features), \textbf{Mouse} ($9$), and
\textbf{Pacing} ($5$) views (Table~\ref{tab:mimictrace-summary}). Default
agents and \Browsium without behavior fail AgentShield and score
$0.949$--$1.000$ on every view. CloakBrowser + Humanize clears AgentShield
($0/10$) yet separates deterministically on compressed keyboard holds
($25.5$\,ms vs.\ $104.0$\,ms human; $1.000$ Keyboard C2ST) and on mouse
($0.990$). \DarkAgent matches human key-hold medians ($106.8$--$110.8$\,ms)
but carries a heavier upper tail on short, chord-heavy fields ($0.936$--$0.945$
Keyboard C2ST).

\noindent\textbf{Mouse view and the action boundary.}
The Mouse view isolates an action-boundary artifact that isolated trajectory
corpora cannot observe. Without pre-click pause calibration, live \MouseGen
matches form movement speed ($\mathrm{AUC}_{\pm}{=}0.527$; Pacing $0.477$) yet
scores $0.986\pm0.030$ Mouse C2ST because \texttt{mouseDown} fires $16.0$\,ms
after pointer arrival versus $58.0$\,ms for humans
($\mathrm{AUC}_{\pm}{=}1.000$). Sampling the pre-click pause from $3{,}110$
click movements across $43$ browser-disjoint \FPAgent human groups ($47.2$\,ms
training median; zero AgentShield sessions used) aligns form pauses ($60.5$\,ms
vs.\ $58.0$\,ms, $\mathrm{AUC}_{\pm}{=}0.605$) over $10/10$ completions with
$0/10$ AgentShield flags, lowering live Mouse C2ST to $0.803\pm0.053$
($p{=}0.030$ vs.\ CloakBrowser + Humanize) while Pacing remains
indistinguishable from the human permutation null ($0.405\pm0.075$,
$p{=}0.707$). Smooth trajectories are therefore insufficient unless the
boundary where motion becomes a click is calibrated as well.

\input{table/mimictrace-channels.tex}

\subsection{Browser and Network Channels: White-Box Audit}
\label{sec:mimictrace-channels}

\noindent\textbf{Audit design.}
Commercial bot services return opaque verdicts without exposing which signal
fired. \MimicTrace instead audits the browser and network surfaces with a
white-box detector built strictly from wire-order HTTP request headers and
standard client-side DOM, WebGL, Canvas, audio, screen, and locale attributes,
with no commercial oracle and no IP, ASN, or geolocation data. Passive
features form four blocks: \emph{network} ($42$ wire-header features),
\emph{browser surface} ($95$ attribute features), \emph{cross-channel
consistency} ($41$ rules: $28$ invariants a self-consistent browser cannot
violate and $11$ headless/container signals), and optional
\emph{human-reference} novelty digests ($23$ features). Unlike raw surface
values, cross-channel contradictions indicate spoofing regardless of the host.

\noindent\textbf{Runtime and WebAssembly integrity.}
Passive attributes are read in a single top-window realm, so main-world
JavaScript getter overrides can satisfy them without engine support. To test
whether a persona is enforced by the engine rather than painted over it,
\MimicTrace adds an $88$-feature \texttt{runtime\_integrity} probe ($48$
descriptors, $26$ invariants, $12$ signals, $2$ counts) across three
boundaries: (i)~a $15$-module WebAssembly feature ladder and the IEEE-754
\texttt{f32.sub(inf, inf)} CPU default-NaN sign joined against
\texttt{userAgentData.architecture}, JS typed arrays, and engine error
dialects; (ii)~native builtin provenance via \texttt{toString},
\texttt{Reflect.construct}, WebIDL brand-check \texttt{TypeError}s, and
call-stack interposition; and (iii)~realm coherence across the top window, a
fresh hidden iframe, and a web worker. Across $13$ stock Windows launches
(Chrome~157, Edge~157, Playwright Chromium~149 and Firefox~150), $0/26$
invariants fire, whereas spoofing controls trigger the expected
engine-dialect, feature-ladder, WebIDL brand-check, and worker-mismatch
invariants. Because \Browsium applies its persona inside Blink rather than
wrapping main-world getters, all $48$ rebuilt \Browsium sessions trigger
$0/26$ invariants and $0/12$ signals (Table~\ref{tab:mimictrace-channels}).

\noindent\textbf{Harness hygiene.}
To rule out collection leakage across corpora, headers enter only through a
15-name browser allowlist, verified bit-identical after stripping and
poisoning excluded headers (\texttt{Host}, \texttt{Cookie}, \texttt{X-*},
\texttt{ASN}, \texttt{City}) across all $7{,}728$ raw \FPAgent records
($7{,}719$ with complete attributes: $546$ humans, $7{,}173$ agents) and all
honeysite sessions ($0$ failures). Without this filter, a logistic regression
given only the \emph{names} of excluded headers separates \FPAgent agents at
$1.000$ ROC-AUC because server-side \texttt{ASN} and \texttt{City} headers
accompany every agent session.

\noindent\textbf{Device-holdout collapse (Protocol~1).}
Comparing $546$ \FPAgent humans against $7{,}173$ agents under 5-fold
browser-group-disjoint CV reaches $0.980$ ROC-AUC on all $178$ environment
features (LogReg; $0.977$ leave-one-family-out), which appears near-perfect.
Yet the seven agent families run on only ten browser groups and seven devices.
Holding out entire \emph{devices} collapses all environment features to
$0.618$ LogReg and browser surface alone to $0.540$. Cross-channel consistency
alone survives at $0.774$ LogReg ($0.742$ XGBoost), driven by the families
that contradict themselves: ChatGPT Agent ($0.984$), Manus ($0.984$), and
Skyvern ($0.885$). The apparent $0.980$ accuracy was largely cloud-VM
memorization.

\noindent\textbf{Zero-shot transfer and invariants (Protocol~2).}
We next fit detectors on \FPAgent alone ($\le 5\%$ FPR on $155$ held-out
\FPAgent humans) and score $112$ honeysite sessions across ten stacks: $48$
sessions on rebuilt \Browsium (intersecting advertised persona WebGL
extensions with active backend support and defaulting to hardware D3D11
rendering across full \DarkAgent and its three ablations) plus $64$ sessions
across six baseline stacks (Table~\ref{tab:mimictrace-channels}). The
\emph{browser surface} XGBoost scores every honeysite stack below held-out
humans ($0.245$--$0.407$ AUC), confirming VM memorization. Named invariants,
by contrast, fire on $0/546$ \FPAgent humans and $0/48$ rebuilt \Browsium
sessions (with $0/48$ \texttt{canvas\textasciitilde gpu} conflicts), while
catching $12/15$ Camoufox sessions (foreign-OS fonts and GPU; $15/15$
\texttt{Accept-Language} vs.\ \texttt{Intl}), $12/12$ Patchright sessions
(unreduced UA, missing \texttt{window.chrome} and \texttt{Accept-Language}),
$995/995$ ChatGPT Agent sessions, and $959/988$ Manus sessions. CloakBrowser +
Humanize triggers $0/12$ invariants but is flagged $12/12$ by
reference-augmented XGBoost because its randomized audio and canvas digests
never occur among real human devices.

\subsection{Multi-Channel Fusion and Adaptive Transfer}
\label{sec:informed-defender}

\noindent\textbf{Channel-wise fusion.}
Because individual channels fail on different stacks, combining them via an
independent channel-wise \textsc{or} over the reference-augmented environment
model, behavioral random forest, and white-box invariants flags $99/112$
honeysite sessions at $2.58\%$ held-out human FPR
(Section~\ref{sec:limitations} discusses transfer across hosts): $12/12$
CloakBrowser + Humanize, $15/15$ Camoufox, $12/12$ Patchright, $12/12$
nodriver, $12/12$ undetected-chromedriver, and all $36/36$ partial \Browsium
ablations on behavior alone, while full \DarkAgent drops to $0/12$
(Table~\ref{tab:mimictrace-channels}).

\noindent\textbf{Transfer to unseen stealth families.}
Under 3-seed leave-one-stealth-family-out evaluation against unseen human
device groups using count-free rate/kinematics plus cross-channel and
reference features ($3.2\%$--$7.8\%$ test FPR), holding out \Browsium leaves
\DarkAgent undetected ($0/12$, $0.536$ AUC), whereas CloakBrowser ($0.905$
AUC, $33.3\%$ detected), Camoufox ($0.945$, $73.3\%$), and Patchright
($0.962$, $66.7\%$) remain separable. The one live-session signal that
survives every protocol is cross-action planning cadence on
\texttt{dynamicForm} ($3.22$\,s vs.\ $4.72$\,s human).

\subsection{Discussion and Limitations}
\label{sec:limitations}

\noindent\textbf{Task and collector transfer.}
Behavioral distributions and environment digests depend on task structure and
on how telemetry is collected. Sampling-rate differences between collectors
($16.4$\,ms pointer polling in \FPAgent vs.\ $9$\,ms in Bo\u{g}azi\c{c}i) and
domain differences between free-text sentences and short form fields shift
feature distributions, which is why the same frozen \MouseGen scores $0.7349$
on its training recorder and $0.9917$ across recorders, and why \KeyboardGen
scores $0.6809$ on Aalto sentences and $0.936$ on chord-heavy form fields.
Cross-dataset environment comparisons between our local honeysite and the
released \FPAgent human logs likewise span distinct host environments, and
AgentShield's released human baseline provides $11$ reference
sessions~\cite{agentshield}. We bound these collection effects by pairing
matched-task C2ST, which holds task and recorder fixed, with cross-channel and
runtime invariants that are host-independent by construction and fire on
$0/546$ \FPAgent humans.

\noindent\textbf{Co-evolution of evasion and detection.}
Live anti-bot measurements on Stealth Bench~V1 capture deployed vendor
policies at the time of evaluation (an $80$-task snapshot from August~21,
2026), and browser execution digests evolve across engine releases, so both
call for periodic re-measurement. More broadly, our findings show that closing
single-channel gaps relocates rather than eliminates defensive signal. As
stealthy browsers enforce engine-level coherence and generative models match
within-action motor statistics, effective defenses shift toward cross-channel
invariants, multi-realm runtime execution checks, and reasoning-induced
cross-action latency across dynamic workflows ($3.22$\,s vs.\ $4.72$\,s on
\texttt{dynamicForm}). \MimicTrace records all of these channels jointly so
that this shift can be measured as both sides evolve.

==> table/mimicgauge-extended.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Full extended detector: human and agent evaluation.}
Each entry gives flagged sessions $k$ / scored sessions $n$ (\%).
The human row measures false positives; agent rows measure detection,
all at the same human-calibrated threshold ($\alpha=\text{TBD}$).
Existing agent logs are rescored where eligible. TBD marks pending measurements.}

\label{tab:mimicgauge-extended}
\small
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\columnwidth}{@{}>{\raggedright\arraybackslash}Xr@{}}
\toprule
\rowcolor{DAPale}
\DAhead{Configuration} & \DAhead{Flagged $k/n$ (\%)} \\
\midrule
Held-out humans & \textcolor{DAWarn}{TBD} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Browser baselines: default behavior}} \\
Chrome / Chromium & \textcolor{DAWarn}{TBD} \\
Firefox & \textcolor{DAWarn}{TBD} \\
Camoufox & \textcolor{DAWarn}{TBD} \\
Patchright & \textcolor{DAWarn}{TBD} \\
CloakBrowser & \textcolor{DAWarn}{TBD} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Browser--behavior and component comparisons}} \\
Chromium, full \Behavium & \textcolor{DAWarn}{TBD} \\
Chromium, \MouseGen only & \textcolor{DAWarn}{TBD} \\
Chromium, \KeyboardGen only & \textcolor{DAWarn}{TBD} \\
\Browsium, no behavior & \textcolor{DAWarn}{TBD} \\
\Browsium, full \Behavium (\DarkAgent) & \textcolor{DAWarn}{TBD} \\
\Browsium, \MouseGen only & \textcolor{DAWarn}{TBD} \\
\Browsium, \KeyboardGen only & \textcolor{DAWarn}{TBD} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Public mimickers}} \\
CloakBrowser + Humanize & \textcolor{DAWarn}{TBD} \\
Chromium + Ghost Cursor & \textcolor{DAWarn}{TBD} \\
Chromium + HumanTyping & \textcolor{DAWarn}{TBD} \\
\Browsium + Ghost Cursor & \textcolor{DAWarn}{TBD} \\
\Browsium + HumanTyping & \textcolor{DAWarn}{TBD} \\
\Browsium + Ghost Cursor + HumanTyping & \textcolor{DAWarn}{TBD} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Additional GUI agents (configurations TBD)}} \\
ChatGPT & \textcolor{DAWarn}{TBD} \\
Claude & \textcolor{DAWarn}{TBD} \\
\bottomrule
\end{tabularx}
\end{table}


==> table/webcloak.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Preliminary WebCloak content-recovery results.}
Exact recovery of all three image URLs (\%) over $N=30$ trials per
decoder and condition. Stage-1 uses structural obfuscation; Stage-2 uses
a semantic decoy. The uncloaked page is the control.}
\label{tab:webcloak}
\small
\setlength{\tabcolsep}{3.6pt}
\begin{tabularx}{\columnwidth}{@{}>{\raggedright\arraybackslash}Xrrr@{}}
\toprule
\rowcolor{DAPale}
\DAhead{Decoder} & \DAhead{Uncloaked} & \DAhead{Stage-1} & \DAhead{Stage-2} \\
\midrule
\rowcolor{DASoft}
\multicolumn{4}{@{}l}{\textcolor{DAAccent}{\textit{DarkAgent deterministic extractor}}} \\
Extractor (ours) & \textbf{100} & \textbf{100} & \textbf{100} \\
\midrule
\rowcolor{DASoft}
\multicolumn{4}{@{}l}{\textcolor{DAAccent}{\textit{OpenAI (gpt-4o-mini)}}} \\
Naive markdown          & 90  & 3 & 57 \\
Crawl4AI-style markdown & 100 & 0 & 100 \\
Decoy-aware markdown    & 100 & 0 & 100 \\
Raw HTML \texttt{src}   & 100 & 0 & 100 \\
Deobfuscate prompt      & 63  & 3 & 60 \\
\midrule
\rowcolor{DASoft}
\multicolumn{4}{@{}l}{\textcolor{DAAccent}{\textit{Gemini (3.6-flash)}}} \\
Naive markdown          & 97  & 0 & 100 \\
Crawl4AI-style markdown & 100 & 0 & 100 \\
Decoy-aware markdown    & 100 & 0 & 100 \\
Raw HTML \texttt{src}   & 100 & 0 & 100 \\
Deobfuscate prompt      & 100 & 73 & 100 \\
\midrule
\rowcolor{DASoft}
\multicolumn{4}{@{}l}{\textcolor{DAAccent}{\textit{Live agents on stock Chromium}}} \\
Browser Use / gpt-4.1          & 100 & 0  & 73 \\
Browser Use / gemini-3.5-flash & 87  & 53 & 100 \\
Browser Use / gemini-3.6-flash & 100 & 13 & 100 \\
Skyvern                        & 0   & 0  & 0 \\
\bottomrule
\end{tabularx}
\end{table}

